Two New Upper Bounds for the Maximum k-plex Problem

A k-plex in a graph is a vertex set where each vertex is non-adjacent to at most k vertices (including itself) in this set, and the Maximum k-plex Problem (MKP) is to find the largest k-plex in the graph. As a practical NP-hard problem, MKP has many important real-world applications, such as the analysis of various complex networks. Branch-and-bound (BnB) algorithms are a type of well-studied and effective exact algorithms for MKP. Recent BnB MKP algorithms involve two kinds of upper bounds based on graph coloring and partition, respectively, that work in different perspectives and thus are complementary with each other. In this paper, we first propose a new coloring-based upper bound, termed Relaxed Graph Color Bound (RelaxGCB), that significantly improves the previous coloring-based upper bound. We further propose another new upper bound, termed RelaxPUB, that incorporates RelaxGCB and a partition-based upper bound in a novel way, making use of their complementarity. We apply RelaxGCB and RelaxPUB to state-of-the-art BnB MKP algorithms and produce eight new algorithms. Extensive experiments using diverse k values on hundreds of instances based on dense and massive sparse graphs demonstrate the excellent performance and robustness of our proposed methods.

==> tabs/table-Instances.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
\centering
\footnotesize
\scalebox{0.8}{\begin{tabular}{lrrrr|rrrr|rrrr} \toprule
\multirow{2}{*}{Instance} & \multicolumn{2}{c}{Cask-Maplex} & \multicolumn{2}{c|}{Maplex}    & \multicolumn{2}{c}{SeesawMKP}  & \multicolumn{2}{c|}{DiseMKP} & \multicolumn{2}{c}{Seesaw-kPlexS} & \multicolumn{2}{c}{kPlexS}     \\ \cline{2-13} 
                          & Branches        & Time          & Branches       & Time         & Branches       & Time          & Branches   & Time           & Branches         & Time           & Branches       & Time          \\ \hline
%2nd DIMACS                &                 &               &                &              &                &               &            &                &                  &                &                &               \\ \hline
brock200-2                & \textbf{6.808}  & \textbf{4.62} & 43.75          & 5.81         & \textbf{1.080} & 3.69          & 7.329      & \textbf{1.93}  & \textbf{0.843}   & \textbf{50.6}  & 2.811          & 153           \\
brock200-3                & \textbf{62.28}  & \textbf{38.4} & 790.8          & 108          & \textbf{7.393} & \textbf{27.2} & 85.88      & 28.4           & \textbf{8.343}   & \textbf{295}   & 52.35          & 1615          \\
brock200-4                & \textbf{171.9}  & \textbf{184}  & 4015           & 577          & \textbf{12.60} & \textbf{60.7} & 279.6      & 109            & \textbf{23.84}   & \textbf{694}   & -              & -             \\
C125-9                    & \textbf{100.4}  & \textbf{281}  & -              & -            & \textbf{15.32} & \textbf{86.4} & -          & -              & \textbf{24.56}   & \textbf{152}   & -              & -             \\
hamming6-2                & \textbf{0.022}  & \textbf{0.05} & 64.94          & 8.51         & \textbf{0.013} & \textbf{0.08} & 31.65      & 7.47           & \textbf{0.032}   & \textbf{0.10}  & 3.657          & 15.9          \\
johnson8-4-4              & \textbf{2.534}  & \textbf{1.08} & 28.06          & 3.13         & \textbf{1.329} & 1.45          & 6.858      & \textbf{1.25}  & \textbf{0.920}   & \textbf{3.30}  & 3.538          & 15.5          \\
keller4                   & \textbf{31.57}  & \textbf{30.1} & 1273           & 182          & \textbf{2.666} & \textbf{9.66} & 69.11      & 22.3           & \textbf{3.961}   & \textbf{85.1}  & 92.45          & 1238          \\
MANN-a9                   & \textbf{0.002}  & \textbf{0.00} & 0.360          & 0.07         & \textbf{0.073} & \textbf{0.09} & 0.646      & 0.16           & \textbf{0.037}   & \textbf{0.04}  & 1.012          & 0.56          \\
san200-0-7-2              & \textbf{0.413}  & \textbf{1.19} & 5.893          & 1.85         & -              & -             & -          & -              & \textbf{383.8}   & \textbf{724}   & -              & -             \\
san200-0-9-1              & \textbf{0.050}  & \textbf{0.84} & -              & -            & \textbf{0.003} & \textbf{0.14} & -          & -              & \textbf{0.024}   & \textbf{0.70}  & -              & -             \\
san200-0-9-2              & \textbf{62.17}  & \textbf{487}  & -              & -            & \textbf{114.9} & \textbf{550}  & -          & -              & \textbf{104.1}   & \textbf{375}   & -              & -             \\
san400-0-5-1              & \textbf{1.690}  & \textbf{5.07} & -              & -            & \textbf{405.2} & \textbf{462}  & -          & -              & \textbf{135.6}   & \textbf{864}   & -              & -             \\
sanr200-0-7               & \textbf{516.6}  & \textbf{538}  & -              & -            & \textbf{40.59} & \textbf{192}  & 1130   & 500            & \textbf{66.05}   & \textbf{1734}  & -              & -             \\ %\hline
%Real-world                &                 &               &                &              &                &               &            &                &                  &                &                &               \\ \hline
soc-BlogCatalog           & -               & -             & -              & -            & \textbf{18.86} & \textbf{1102} & -          & -              & -                & -              & -              & -             \\
soc-buzznet               & \textbf{70.90}  & \textbf{561}  & -              & -            & \textbf{2.275} & \textbf{97.5} & -          & -              & -                & -              & -              & -             \\
soc-digg                  & \textbf{1.632}  & \textbf{89.4} & -              & -            & \textbf{0.207} & \textbf{2.58} & 250.2      & 157            & \textbf{0.470}   & \textbf{91.8}  & -              & -             \\
socfb-Duke14              & \textbf{0.315}  & \textbf{1.01} & 195.6          & 45.0         & \textbf{0.046} & \textbf{3.07} & 226.4      & 131            & \textbf{0.110}   & \textbf{4.45}  & 1.046          & 36.6          \\
socfb-Indiana             & \textbf{0.021}  & \textbf{0.14} & 716.0          & 313          & \textbf{0.046} & \textbf{4.41} & 141.1      & 105            & \textbf{0.013}   & \textbf{1.99}  & \textbf{0.013} & 2.30          \\
socfb-Texas84             & \textbf{0.035}  & \textbf{0.13} & -              & -            & \textbf{0.061} & \textbf{4.16} & 391.3      & 293            & \textbf{0.055}   & \textbf{2.45}  & 0.240          & 3.83          \\
socfb-UF                  & \textbf{0.033}  & \textbf{0.37} & -              & -            & \textbf{0.161} & \textbf{5.70} & 17.92      & 12.8           & \textbf{0.094}   & \textbf{2.19}  & 0.190          & 3.31          \\
socfb-UIllinois           & \textbf{0.064}  & \textbf{2.05} & -              & -            & \textbf{0.015} & \textbf{7.83} & 31.61      & 21.6           & \textbf{0.022}   & \textbf{2.15}  & 0.023          & 2.63          \\
soc-flixster              & \textbf{0.159}  & \textbf{0.46} & 373.5          & 68.3         & \textbf{0.015} & \textbf{7.83} & 31.61      & 21.6           & \textbf{0.052}   & \textbf{3.95}  & 1.908          & 27.1          \\
soc-FourSquare            & 77.43           & 815           & \textbf{56.71} & \textbf{313} & \textbf{0.046} & \textbf{32.2} & -          & -              & \textbf{0.056}   & \textbf{12.6}  & 0.067          & 13.0          \\
soc-LiveMocha             & \textbf{2.907}  & \textbf{6.69} & 41.38          & 14.8         & \textbf{0.231} & \textbf{9.03} & 7.819      & 9.44           & \textbf{0.114}   & \textbf{21.4}  & 0.693          & 45.4          \\
soc-orkut                 & -               & -             & -              & -            & -              & -             & -          & -              & \textbf{0.435}   & \textbf{301}   & -              & -             \\
soc-slashdot              & \textbf{0.038}  & \textbf{0.09} & 42.13          & 6.19         & \textbf{0.008} & \textbf{0.42} & 2.544      & 1.24           & \textbf{0.014}   & \textbf{0.28}  & 0.092          & 1.15          \\
tech-as-skitter           & \textbf{0.011}  & \textbf{0.07} & 443.9          & 187          & \textbf{0.018} & \textbf{16.6} & 660.7      & 544            & \textbf{0.001}   & 4.58           & \textbf{0.001} & \textbf{4.09} \\
tech-WHOIS                & \textbf{0.020}  & \textbf{0.09} & -              & -            & \textbf{0.009} & \textbf{0.19} & 112.1      & 90.5           & \textbf{0.030}   & \textbf{0.19}  & 0.407          & 3.95     \\ \bottomrule   
\end{tabular}}
\caption{Comparison on 28 representative MKP instances with $k = 2$. The branches are in $10^5$ and time is in seconds.}
\label{table-Instances}
\end{table*}

==> tabs/table2.tex <==
\begin{table*}[!t]
\centering
\footnotesize
\scalebox{0.84}
{\begin{tabular}{lrrrr|rrrr|rrrr|rrrr} \toprule
\multirow{2}{*}{Instance} & \multicolumn{2}{c}{Relax-Maplex} & \multicolumn{2}{c|}{Maplex}      & \multicolumn{2}{c}{Seesaw-kPlexS} & \multicolumn{2}{c|}{kPlexS}      & \multicolumn{2}{c}{Seesaw-MKP}   & \multicolumn{2}{c|}{DiseMKP} & \multicolumn{2}{c}{Seesaw-KPLEX} & \multicolumn{2}{c}{KPLEX} \\ \cline{2-17}
                          & Tree            & Time            & Tree           & Time           & Tree            & Time            & Tree           & Time           & Tree           & Time           & Tree     & Time             & Tree            & Time           & Tree    & Time            \\ \hline
brock200-3                & \textbf{62.28}  & \textbf{41.97}  & 790.8          & 107.8          & \textbf{8.343}  & \textbf{292.0}  & 52.35          & 1615       & \textbf{7.393} & \textbf{22.66} & 85.88    & 28.40            & \textbf{27.43}  & \textbf{34.63} & 225.2   & 80.52           \\
brock200-4                & \textbf{171.9}  & \textbf{131.6}  & 4015           & 576.9          & \textbf{23.84}  & \textbf{695.8}  & -              & -              & \textbf{12.60} & \textbf{48.76} & 279.6    & 109.4            & \textbf{68.81}  & \textbf{84.81} & 780.2   & 250.0           \\
C125-9                    & \textbf{100.4}  & \textbf{225.2}  & -              & -              & \textbf{24.56}  & \textbf{162.8}  & -              & -              & \textbf{15.32} & \textbf{75.64} & -        & -                & \textbf{29.61}  & \textbf{37.93} & -       & -               \\
hamming6-2                & \textbf{0.022}  & \textbf{0.039}  & 64.94          & 8.512          & \textbf{0.032}  & \textbf{0.108}  & 3.657          & 15.89          & \textbf{0.013} & \textbf{0.044} & 31.65    & 7.467            & \textbf{0.023}  & \textbf{0.032} & 1.761   & 0.361           \\
johnson8-4-4              & \textbf{2.534}  & \textbf{1.175}  & 28.06          & 3.130          & \textbf{0.920}  & \textbf{3.870}  & 3.538          & 15.46          & \textbf{1.329} & \textbf{1.252} & 6.858    & \textbf{1.252}   & \textbf{1.770}  & \textbf{1.023} & 11.93   & 1.838           \\
keller4                   & \textbf{31.57}  & \textbf{27.49}  & 1273           & 182.3          & \textbf{3.961}  & \textbf{87.18}  & 92.45          & 1238           & \textbf{2.666} & \textbf{8.339} & 69.11    & 22.33            & \textbf{19.29}  & \textbf{17.38} & 562.6   & 105.3           \\
MANN-a9                   & \textbf{0.002}  & \textbf{0.006}  & 0.360          & 0.067          & \textbf{0.037}  & \textbf{0.054}  & 1.012          & 0.560          & \textbf{0.073} & \textbf{0.067} & 0.646    & 0.156            & \textbf{0.006}  & \textbf{0.004} & 0.026   & 0.009           \\
MANN-a27                  & \textbf{1.395}  & \textbf{112.1}  & -              & -              & -               & -               & -              & -              & -              & -              & -        & -                & \textbf{0.924}  & \textbf{8.902} & -       & -               \\
p-hat300-2                & \textbf{54.33}  & \textbf{98.94}  & -              & -              & \textbf{4.143}  & \textbf{144.5}  & -              & -              & \textbf{1.339} & \textbf{9.349} & 865.6    & 542.8            & \textbf{389.9}  & \textbf{1083}  & -       & -               \\
san200-0-7-1              & \textbf{2.414}  & \textbf{6.216}  & -              & -              & -               & -               & -              & -              & -              & -              & -        & -                & \textbf{1.918}  & \textbf{3.859} & -       & -               \\
san200-0-7-2              & \textbf{0.413}  & \textbf{1.768}  & 5.893          & 1.851          & \textbf{383.8}  & \textbf{720.3}  & -              & -              & -              & -              & -        & -                & \textbf{0.426}  & \textbf{1.584} & -       & -               \\
san200-0-9-1              & \textbf{0.050}  & \textbf{0.622}  & -              & -              & \textbf{0.024}  & \textbf{0.660}  & -              & -              & \textbf{0.003} & \textbf{0.108} & -        & -                & \textbf{0.057}  & \textbf{0.619} & 64.21   & 27.33           \\
san200-0-9-2              & \textbf{62.17}  & \textbf{406.3}  & -              & -              & \textbf{104.1}  & \textbf{373.4}  & -              & -              & \textbf{114.9} & \textbf{456.3} & -        & -                & \textbf{11.88}  & \textbf{59.84} & -       & -               \\
san400-0-5-1              & \textbf{1.690}  & \textbf{5.300}  & -              & -              & \textbf{135.6}  & \textbf{904.8}  & -              & -              & \textbf{405.2} & \textbf{350.4} & -        & -                & \textbf{1.878}  & \textbf{11.64} & -       & -               \\
sanr200-0-7               & \textbf{516.6}  & \textbf{457.9}  & -              & -              & \textbf{66.05}  & \textbf{1656}   & -              & -              & \textbf{40.59} & \textbf{169.7} & 1130     & 499.6            & \textbf{171.7}  & \textbf{206.6} & 2681    & 752.0           \\
soc-BlogCatalog           & -               & -               & -              & -              & -               & -               & -              & -              & \textbf{18.86} & \textbf{974.5} & -        & -                & -               & -              & -       & -               \\
soc-buzznet               & \textbf{70.90}  & \textbf{464.9}  & -              & -              & -               & -               & -              & -              & \textbf{2.275} & \textbf{91.52} & -        & -                & \textbf{27.04}  & \textbf{1097}  & 414.2   & 1528            \\
soc-digg                  & \textbf{1.632}  & \textbf{60.94}  & -              & -              & \textbf{0.470}  & \textbf{83.93}  & -              & -              & \textbf{43.92} & \textbf{1765}  & -        & -                & \textbf{1.616}  & \textbf{93.13} & 34.89   & 362.8           \\
socfb-Duke14              & \textbf{0.315}  & \textbf{1.084}  & 195.6          & 45.05          & \textbf{0.110}  & \textbf{4.397}  & 1.046          & 36.58          & \textbf{0.207} & \textbf{2.270} & 250.2    & 157.0            & \textbf{0.281}  & \textbf{2.403} & 1.598   & 2.957           \\
socfb-Indiana             & \textbf{0.021}  & \textbf{0.234}  & 716.0          & 312.8          & \textbf{0.013}  & \textbf{1.928}  & 0.013          & 2.304          & \textbf{0.046} & \textbf{3.507} & 226.4    & 130.5            & \textbf{0.024}  & \textbf{1.637} & 0.025   & 1.751           \\
socfb-OR            & \textbf{0.010}           & \textbf{0.014}            & 30.35 & 4.106 & \textbf{0.018}  & \textbf{0.643}           & 0.032          & 0.702 & \textbf{0.016} & \textbf{1.115} & 1.798        & 1.453                & \textbf{0.020}  & \textbf{0.382} & 0.050   & 0.507           \\
socfb-Texas84             & \textbf{0.035}  & \textbf{0.135}  & -              & -              & \textbf{0.055}  & \textbf{2.417}  & 0.240          & 3.828          & \textbf{0.046} & \textbf{3.026} & 141.1    & 104.6            & \textbf{0.066}  & 2.502          & 0.151   & \textbf{1.780}  \\
socfb-UF                  & \textbf{0.033}  & \textbf{0.317}  & -              & -              & \textbf{0.094}  & \textbf{2.012}  & 0.190          & 3.310          & \textbf{0.061} & \textbf{3.122} & 391.3    & 292.7            & \textbf{0.107}  & \textbf{1.741} & 0.234   & 1.850           \\
socfb-UIllinois           & \textbf{0.064}  & \textbf{1.425}  & -              & -              & \textbf{0.022}  & \textbf{2.224}  & 0.023          & 2.628          & \textbf{0.161} & \textbf{4.636} & 17.92    & 12.81            & \textbf{0.024}  & \textbf{1.774} & 0.027   & 1.845           \\
soc-flixster              & \textbf{0.159}  & \textbf{0.435}  & 373.5          & 68.29          & \textbf{0.052}  & \textbf{3.776}  & 1.908          & 27.13          & \textbf{0.015} & \textbf{6.596} & 31.61    & 21.65            & \textbf{0.142}  & \textbf{1.478} & 0.819   & 1.739           \\
%soc-FourSquare            & 77.43           & 1046            & \textbf{56.71} & \textbf{313.3} & \textbf{0.056}  & 13.11           & 0.067          & \textbf{12.98} & \textbf{0.046} & \textbf{36.93} & -        & -                & \textbf{0.093}  & \textbf{15.07} & 0.150   & 15.59           \\
soc-LiveMocha             & \textbf{2.907}  & \textbf{5.419}  & 41.38          & 14.84          & \textbf{0.114}  & \textbf{22.21}  & 0.693          & 45.43          & \textbf{0.231} & \textbf{7.060} & 7.819    & 9.442            & \textbf{0.842}  & \textbf{8.402} & 3.582   & 8.933           \\
soc-orkut                 & -               & -               & -              & -              & \textbf{0.435}  & \textbf{295.2}  & -              & -              & -              & -              & -        & -                & \textbf{1.445}  & \textbf{291.4} & 49.47   & 301.4           \\
soc-slashdot              & \textbf{0.038}  & \textbf{0.079}  & 42.13          & 6.185          & \textbf{0.014}  & \textbf{0.296}  & 0.092          & 1.151          & \textbf{0.008} & \textbf{0.290} & 2.544    & 1.242            & \textbf{0.037}  & \textbf{0.163} & 0.135   & 0.182           \\
tech-as-skitter           & \textbf{0.011}  & \textbf{0.041}  & 443.9          & 187.3          & \textbf{0.001}  & 5.777           & \textbf{0.001} & \textbf{4.085} & \textbf{0.018} & \textbf{19.81} & 660.7    & 544.2            & \textbf{0.001}  & \textbf{0.944} & 0.001   & 1.043           \\
tech-WHOIS                & \textbf{0.020}  & \textbf{0.147}  & -              & -              & \textbf{0.030}  & \textbf{0.205}  & 0.407          & 3.953          & \textbf{0.009} & \textbf{0.109} & 112.1    & 90.50            & \textbf{0.039}  & \textbf{0.142} & 0.100   & 0.166  \\ \bottomrule   
\end{tabular}}
\caption{Comparison on 30 representative MKP instances with $k = 2$. The search tree size is in $10^5$, and the time is in seconds. Better results appear in bold.}
\label{table-Instances}
\end{table*}
